Telling Two Distributions Apart: a Tight Characterization

We consider the problem of distinguishing between two arbitrary black-box distributions defined over the domain [n], given access to $s$ samples from both. It is known that in the worst case O(n^{2/3}) samples is both necessary and sufficient, provided that the distributions have L1 difference of at least {\epsilon}. However, it is also known that in many cases fewer samples suffice. We identify a new parameter, that provides an upper bound on how many samples needed, and present an efficient algorithm that requires the number of samples independent of the domain size. Also for a large subclass of distributions we provide a lower bound, that matches our upper bound up to a poly-logarithmic factor.

==> weights_lemma.tex <==
Now we prove the key lemma that will provide with a way of estimating the likelyhood ratio
\begin{lemma}
   Let $C_P, D_P$ and $C_Q, D_Q$ be the probability masses of subsets of
$\common(\pi P, \pi Q)$ and $\disjoint(\pi P, \pi Q)$ that were
sampled during training phase of $P$ and $Q$ respectively.
Further, let $\numsigs 101 = a$  and $\numsigs 011=b$, and assume $C_P \le C$, $D_P \ge D$,
$C_Q \ge C$ and $D_Q \le D$
Then we have:
$$
 \frac{L(H_1 |~ \numsigs 101=a, \numsigs 011= b)}{L(H_2 | ~\numsigs 011=a, \numsigs 011 b)}  \le (1 + D/C) ^{a - b}
$$
\end{lemma}
\proof{
First of all by lemma \ref{lem:random-to-fixed} we can assume that the set where second and all higher order collisions have occurred
is fixed in advance and we just need to compute the likelyhood ratio of observed configuration of single collisions.
Let us denote all possible orders of how we could have achieve $\numsigs101$ and $\numsigs011$ as $\cal X$.  Then we have:
$$
   \frac{\Pr{\numsigs 101=a, \numsigs 011= b | H_1}}{\Pr{\numsigs 101=a, \numsigs 011= b | H_2}} =
\frac{\sum_{x \in \cal X} \Pr{x | H_1}}{\sum_{x \in \cal X} \Pr{x |  H_2}}
$$
Thus, by lemma \ref{lem:tech-lemma}, it is sufficient  to prove our bounds for each configuration individually. Namely
consider $\{x_i\}$ and $\{y_i\}$  be the indicator variables for whether $i$-th testing sample belongs to $\Train_P$, $\Train_Q$.
Let $C_P^{(i)}, C_Q^{(i)}, D_P^{(i)}, D_Q^{(i)}$,  be the weights of common and disjoint parts of
$\Train_P$, $\Train_Q$ respectively that has not appeared in $\Test$ untli
 $i$-th sample. Then we have:
$$
  \Pr{ \{x_i\}, \{y_i\} | H_1} = \prod(C_P^{(i)} + D_P^{(i)})^{x_i}(C_Q^{(i)})^{y_i}
(1 - C_P^{(i)} - C_Q^{(i)} - D_P^{(i)})^{1-x_i-y_i}
$$
where we used the  fact that probability of having $x_i=1, y_i=0$ is
$C_P^{(i)} + D_P^{(i)}$, probability of $y_i=1, x_i=0$ is
$C_Q^{(i)}$, probability of $x_i=0,y_i=0$ is $C_P^{(i)} - C_Q^{(i)} - D_P^{(i)}$
and finally  $x_i=1, y_1=1$ is impossible. Similarly we have:
$$
  \Pr{ \{x_i\}, \{y_i\} | H_2} = \prod(C_P^{(i)})^{x_i}(D_Q^{(i)} + C_Q^{(i)})^{y_i} (1 - C_P^{(i)} - C_Q^{(i)} - D_Q^{(i)})^{1-x_i-y_i}
$$
therefore we have:
$$
\frac{\Pr{ \{x_i\}, \{y_i\} | H_1} }
{  \Pr{ \{x_i\}, \{y_i\} | H_2}} =
\frac{(\frac{C_P^{(i)}+D_P^{(i)}}{C_P^{(i)}})^a}
{(\frac{C_Q^{(i)}+D_Q^{(i)}}{C_Q^{(i)}})^b}
$$


wNote that since no element of $P$ and $Q$ has a high probability we have $C$  Then we have:
$$
  \Pr{\{t_i\}, \{y_i\}}
$$
index where we obverved a new unique collision with $\Train_P$.
Let $C_P^{(i)}, C_Q^{(i)}$,  be the weights indicating the weight of common part of $\Train_P$, $\Train_Q$
which has not been selected prior to step $i$. Then we have
$$
 \Pr{l_1, \dots l_i} = \Pr{l_1} \Pr{l_2| l_1} \dots \Pr{l_a | l_1, l_2, \dots l_{a-1}} =f
$$

}

